Recursive Top-Down Production for Sentence Generation with Latent Trees

We model the recursive production property of context-free grammars for natural and synthetic languages. To this end, we present a dynamic programming algorithm that marginalises over latent binary tree structures with $N$ leaves, allowing us to compute the likelihood of a sequence of $N$ tokens under a latent tree model, which we maximise to train a recursive neural function. We demonstrate performance on two synthetic tasks: SCAN (Lake and Baroni, 2017), where it outperforms previous models on the LENGTH split, and English question formation (McCoy et al., 2020), where it performs comparably to decoders with the ground-truth tree structure. We also present experimental results on German-English translation on the Multi30k dataset (Elliott et al., 2016), and qualitatively analyse the induced tree structures our model learns for the SCAN tasks and the German-English translation task.

==> introduction.tex <==
\section{Introduction}
Distributed representations have successfully been employed in language models \cite{bengio2003neural} to deal with the curse of dimensionality.
Since the advent of neural language models, there has been considerable improvement in natural language processing and generation tasks.

Despite its recent successes, recurrent neural networks (RNNs; \citealt{elman1990finding}) fail at tasks that explicitly require and test compositional behavior \citep{lake2017generalization,loula2018rearranging}.
\citet{hupkes2019compositionality} also showed that transformer-based models \citep{devlin2018bert,yang2019xlnet}, while having performed spectacularly at NLP tasks recently, may fail to generalise when tested against synthetic data that was generated with compositional phenomena.
It is unclear if these tests will predict larger issues with these current models down the road, but, if hierarchical generation plays a important role in language generation, then the above models have inherent biases in their structure that do not fit the task. Text generation in these models are typically sequential processes: each token is generated one at a time from left to right.

In this paper, we propose a model for generating sentences from a latent tree structure, that aims to reflect natural language syntax. Our method assumes that each token in a sentence is emitted at the leaves of an unobserved, full binary tree. We provide a dynamic programming algorithm to efficiently marginalize over the combinatorial number of latent binary trees.
Our approach parametrises emission probabilities at the leaves and the prior distribution over trees with neural networks (NN).
Each tree is obtained by a recursive NN, where the node embeddings are recursively obtained by splitting the root embedding.

Our approach differ from PCFGs \cite{fu1974syntactic} in several aspects: i) we do not have to specify a finite set of non-terminal symbols and production rules, but now have a uncountably infinite set of them via distributed representations and ii) each (implicit) production rule is embedded in a continuous space which increases the expressivity of the model.
In setting aside symbolic production rules, we lose the ability to use the Inside algorithm~\citep{baker1979trainable} and thus require an alternate means of computing the likelihood of the sequence.

In the next section, we will describe an algorithm that marginalises over latent tree structures under some independence assumptions.
We first introduce these assumptions and show that by introducing the notion of successive leaves, we can efficiently sum over different tree structures. We then introduce the details of the recursive architecture used. Finally, we present the experimental results  of the model in Section~\ref{sec:experiments}.


